InfoBERT: Improving Robustness of Language Models from An Information Theoretic Perspective

Large-scale language models such as BERT have achieved state-of-the-art performance across a wide range of NLP tasks. Recent studies, however, show that such BERT-based models are vulnerable facing the threats of textual adversarial attacks. We aim to address this problem from an information-theoretic perspective, and propose InfoBERT, a novel learning framework for robust fine-tuning of pre-trained language models. InfoBERT contains two mutual-information-based regularizers for model training: (i) an Information Bottleneck regularizer, which suppresses noisy mutual information between the input and the feature representation; and (ii) a Robust Feature regularizer, which increases the mutual information between local robust features and global features. We provide a principled way to theoretically analyze and improve the robustness of representation learning for language models in both standard and adversarial training. Extensive experiments demonstrate that InfoBERT achieves state-of-the-art robust accuracy over several adversarial datasets on Natural Language Inference (NLI) and Question Answering (QA) tasks. Our code is available at https://github.com/AI-secure/InfoBERT.

==> tables/adv_squad.tex <==
\begin{table}[htp!] \setlength{\tabcolsep}{7pt}
%
\scriptsize
\centering
\begin{tabular}{c|l|c|cc}
\toprule
Training & {Regularizer}  & {benign} & {{AddSent}} & {AddOneSent} \\
\midrule
\multirow{2}{*}{\shortstack{Standard \\Training}  }    & Baseline     & \textbf{93.5}/86.9  & 72.9/66.6  & 80.6/74.3 \\
                                                       & InfoBERT     & \textbf{93.5/87.0}  & \textbf{78.5/72.9}  & \textbf{84.6/78.3} \\ 
                                                    %   & +IB          & \textbf{93.9/87.5}  & 77.2/71.4  & 83.8/77.7    \\
                                                    %   & +Local       & 93.7/87.1  & 77.9/72.0  & 83.5/77.2    \\
                                                    %   & +IB+Local    & 93.5/87.0  & \textbf{78.5/72.9}  & \textbf{84.6/78.3} \\ 
                                                       
\midrule
\midrule                                                      
\multirow{3}{*}{\shortstack{Adversarial \\Training}}   & Baseline     & \textbf{93.8}/\textbf{87.3}   & 76.3/70.3  & 82.3/76.2 \\
                                                       & ALUM         & -            & 75.5/69.4  &  81.4/75.9 \\
                                                       & InfoBERT     & 93.7/87.0  &  \textbf{78.0/71.8} &   \textbf{83.6/77.1} \\
                                                    %   & +IB          & 93.7/87.0  &  \textbf{78.0/71.8} &   \textbf{83.6/77.1} \\
                                                    %   & +Local       & 93.6/87.0  &  75.0/68.8 & 81.5/75.2 \\
                                                    %   & +Local+IB    &  \textbf{93.9/87.3} & 75.8/69.5 & 82.9/76.2 \\
\bottomrule   
\end{tabular}
\caption{Robust F1/EM score of RoBERTa$_{\text{Large}}$-based models on the adversarial SQuAD dataset (AddSent and AddOneSent). Models are trained on standard SQuAD 1.0 dataset.} \label{tab:adv_squad}
\end{table}
